MAWSEO: Adversarial Wiki Search Poisoning for Illicit Online Promotion

As a prominent instance of vandalism edits, Wiki search poisoning for illicit promotion is a cybercrime in which the adversary aims at editing Wiki articles to promote illicit businesses through Wiki search results of relevant queries. In this paper, we report a study that, for the first time, shows that such stealthy blackhat SEO on Wiki can be automated. Our technique, called MAWSEO, employs adversarial revisions to achieve real-world cybercriminal objectives, including rank boosting, vandalism detection evasion, topic relevancy, semantic consistency, user awareness (but not alarming) of promotional content, etc. Our evaluation and user study demonstrate that MAWSEO is capable of effectively and efficiently generating adversarial vandalism edits, which can bypass state-of-the-art built-in Wiki vandalism detectors, and also get promotional content through to Wiki users without triggering their alarms. In addition, we investigated potential defense, including coherence based detection and adversarial training of vandalism detection, against our attack in the Wiki ecosystem.

==> 1abstract.tex <==
\begin{abstract}
As a prominent instance of vandalism edits, Wiki search poisoning for illicit promotion is a cybercrime in which the adversary aims at editing Wiki articles to promote illicit businesses through Wiki search results of relevant queries. 
% 
In this paper, we contribute a pioneer investigation that enables such stealthy blackhat SEO on Wiki, called \textit{MAWSEO}. This technique employs adversarial revisions to achieve real-world cybercriminal objectives, including rank boosting, vandalism detection evasion, topic relevancy, semantic consistency, user awareness (but not alarming) of promotional content, etc. 
% 
Our evaluation and user study show that MAWSEO is able to effectively and efficiently generate adversarial vandalism edits, which can bypass state-of-the-art and built-in Wiki vandalism detectors, and also get promotional content through to Wiki users without triggering their alarms.
%
In addition, we investigated potential defense, including coherence based detection and adversarial training of the vandalism detection against our attack in the Wiki ecosystem. 







\ignore{
%The public Wiki system provides a powerful channel for knowledge sharing, integration, and reuse. However, it is struggling to balance between maintenance of open editing and defense against vandalism, where the Wiki article has been edited in a disruptive or malicious manner. 
%
As a prominent instance of vandalism edits, Wiki search poisoning for illicit promotion is a cybercrime in which the adversary aims at editing Wiki articles to promote illicit businesses through Wiki search results of relevant queries. 
%For this purpose, one needs to solve a challenging adversarial revision problem: \ignore{that is, }how to hide \zlsec{edits}\ignore{the editing} from Wiki's vandalism detection and avoid complaints from human users but still capture their attention. 
In this paper, we contribute a pioneer investigation that enables such stealthy blackhat SEO on Wiki, called \textit{MAWSEO}. This technique employs adversarial revisions to achieve real-world cybercriminal objectives, including rank boosting, vandalism detection evasion, topic relevancy, semantic consistency, user awareness (but not alarming) of promotional content, etc. 
%
%More specifically, we propose a multi-task adversarial passage retrieval model, which enables a black-box Wiki search poisoning attack for illicit promotion. A unique strength of this approach is that it transforms the challenging adversarial revision generation task into a passage retrieval task, which can be done efficiently.
%
%\zlsec{We evaluated MAWSEO on illicit online pharmacy promotion.}\ignore{We implemented MAWSEO and evaluated it on the task of illicit online pharmacy promotion.} 
Our evaluation and user study show that MAWSEO is able to effectively and efficiently generate adversarial vandalism edits, which can bypass state-of-the-art and built-in Wiki vandalism detectors, and also get \ignore{the }promotional content through to Wiki users without triggering their alarms.
%
In addition, we investigated potential defense, including coherence based detection and adversarial training of the vandalism detection against our attack in the Wiki ecosystem. 
%
%Our research leads to a new understanding of the threat of Wiki data poisoning for illicit promotion, which we show can be aggravated by adversarial ranking, and identifies potential avenues to mitigate such threats.
}


%The public Wiki system provides a powerful approach for knowledge sharing, integration, and reuse. However, the public Wiki system is struggled to maintain a good balance between open editing and protecting against vandalism edits, where the Wiki page has been edited in a disruptive or malicious manner. 
%As an instance of vandalism edits, Wiki search poisoning for illicit promotion is a kind of cybercrime where the adversary aims at editing the Wiki pages to promote the information of the illicit businesses in Wiki search engine results of relevant queries.

%In this study, we study an innovative blackhat SEO technique, named MAWSEO, on the Wiki system. This technique employs adversarial ranking attack techniques while considering real-world cybercriminal attack objectives, including rank boosting, vandalism detection evasion, semantic consistency, and user awareness (but not alarming) of promotional content, etc. 
% More specifically, we propose a multi-task adversarial passage retrieval model, which enables blackbox Wiki search poisoning attack for illicit promotion. A unique strength of this approach is that it transforms the challenging adversarial revision generation task into a passage retrieval task, which is lightweight, efficient, and evasive.
% We implement MAWSEO and evaluate it on the task of illicit online pharmarcy promotion. The evaluation and user study results show that MAWSEO is able to effectively and efficently generate adversarial vandalism edits, which can bypass state-of-the-art and built-in Wiki vandalism detectors, as well as get the promotional content through Wiki users without triggering their alarms.
%In addition, we study defense methods, including coherence based detection and adversarial training of vandalism detector, against the above illicit promotion approach on Wiki system. 
%Our study enables a better understanding of Wiki data poisoning attack, which is equipped with adversarial ranking attack techniques, for the cybercrime of illicit promotion, and suggests potential avenues to disrupt these threats.


\end{abstract}



\ignore{
The public Wiki system provides a powerful channel for knowledge sharing, integration, and reuse. However, it is struggling to balance between maintenance of open editing and defense against vandalism, where the Wiki page has been edited in a disruptive or malicious manner. 
%
As a prominent instance of vandalism edits, Wiki search poisoning for illicit promotion is a kind of cybercrime where the adversary aims at editing Wiki pages to promote illicit businesses through Wiki search results for relevant queries.

In this paper, we report an innovative technique for blackhat SEO, named MAWSEO, on the Wiki system. This technique employs adversarial ranking attack techniques to achieve real-world cybercriminal objectives, including rank boosting, vandalism detection evasion, semantic consistency, user awareness (but not alarming) of promotional content, etc. 
%
More specifically, we propose a multi-task adversarial passage retrieval model, which enables a black-box Wiki search poisoning attack for illicit promotion. A unique strength of this approach is that it transforms the challenging adversarial revision generation task into a passage retrieval task, which is lightweight, efficient, and evasive.
%
We implement MAWSEO and evaluate it on the task of illicit online pharmacy promotion. Our evaluation and user study show that MAWSEO is able to effectively and efficiently generate adversarial vandalism edits, which can bypass state-of-the-art and built-in Wiki vandalism detectors, as well as get the promotional content through Wiki users without triggering their alarms.
%
In addition, we study defense methods, including coherence based detection and adversarial training of the vandalism detector against the above illicit promotion approach on the Wiki system. 
%
Our study leads to a new understanding of\ignore{about} the threat of Wiki data poisoning for illicit promotion, which we show can be aggravated by adversarial ranking, and suggests potential avenues to mitigate such a threat.
}

==> 8relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}

\noindent\textbf{Illicit online promotion}.
% drug promotion
The flooding of illicit online promotion for business success or misinformation spreading is a worldwide epidemic. Particularly, the abuse of non-prescription and addictive medications fosters the growth of illicit online pharmacies and their\ignore{the development of} drug promotion strategies. McCoy et al. measured the illicit online pharmacies and the pharmaceutical affiliate programs~\cite{mccoy2012pharmaleaks}. Leotiadis et al. analyzed the advertising network of online pharmacies in a four-year study~\cite{leontiadis2014nearly}.
%
The prior work also studied online market promotion of counterfeit luxury goods~\cite{wang2014search}.

% misinformation (wiki) promotion
Recently\ignore{In recent years}, online misinformation promotion has obtained more attention.
Yao et al. studied the attack and defense in online review systems by producing fake reviews with machine-learning methods~\cite{yao2017automated}. 
%
Sharevski et al. tried to inject incorrect knowledge into Wikipedia in a vandalism manner~\cite{sharevski2020wikipediabot}. However, for vandalism edits, those studies designed models based solely on context-relevant word generations or substitutions without considering rank boosting, vandalism detection evasion, or article topic relevancy. 


\noindent\textbf{Search poisoning attack}.
% general search engine strategy
The search poisoning attack has been studied extensively. As a natural and direct strategy, adversaries were found to attack search results by \zlsec{stuffing keywords into victim pages }or injecting promotional content \zlndss{pages} into popular sites in a semantic-inconsistent manner~\cite{liao2016characterizing,liao2016seeking}, \zlndss{cloaking malicious pages with benign pages containing popular search terms~\cite{wang2011cloak}, }or creating many fake web pages targeting trendy keywords~\cite{john2011deseo}.
%
To leverage the functionality of links in search engines, the adversaries used search-redirection and link farms to promote target pages or content~\cite{leontiadis2011measuring,wu2005identifying}. 
%
However, these traditional SEO methods have been deeply studied. The corresponding tools or strategies have been designed against such attacks~\cite{liao2016seeking,leontiadis2011measuring}. 
\zlndss{All known traditional SEO methods gaming search ranking aim at search engines, not open-edit systems like Wiki, under different threat models (see Section~\ref{subsec:threatmodel}): e.g., they require compromising websites to insert content, but do not require \zlndss{topic relevancy,} semantic consistency or detection evasion\ignore{, etc}~\cite{liao2016characterizing,liao2016seeking,john2011deseo,wang2011cloak,leontiadis2011measuring}.}


%Adversarial Ranking Attack
Adversarial learning is the state-of-the-art approach applied for the search poisoning attack, using adversarial examples to attack the ranking algorithms. 
%
Previous adversarial ranking attacks primarily focused on image ranking manipulation~\cite{liu2019afraidqueries,zhou2020adversarial,zhou2021practical}. Researchers proposed methods to generate adversarial image queries, which can lead to incorrect retrieval results~\cite{liu2019afraidqueries,zhou2020adversarial,zhou2021practical}. To disorder the ranking results, attackers also generated adversarial image retrieval candidates to raise or lower the rank of a single candidate~\cite{zhou2020adversarial}.
%
The adversarial attacks on natural language processing models also inspired the study of the vulnerability of text ranking systems facing adversarial learning.
%
Song et al.~\cite{song2020adversarial} proposed a white-box attack to insert semantically \textit{unrelated} texts
into a document for rank boosting.
%
\zlccs{To further attack the black-box ranking system, Liu et al.~\cite{liu2022order} crafted machine-generated trigger texts via a fine-tuned Song's model.\ignore{, which underperforms our approach when faced with the \textit{real-world} black-box ranking system (see Sections~\ref{subsec:promotionEffective} and~\ref{subsec:userstudy}).}
% 
A state-of-the-art approach of the word substitution~\cite{wu2022prada} was also proposed to attack neural ranking systems through replacing important words in the text with their synonyms.}
%
% Goren et al. studied the robustness of learning-to-rank-based relevance ranking functions to adversarial document manipulations~\cite{goren2018ranking}.
%
In contrast to previous studies on adversarial ranking attacks, our work focuses on a real-world cybercrime and its attack goals -- blackhat SEO for promotional infection, where the attackers \textit{disorder the ranking} of a \zlccs{\textit{real-world black-box}} Wiki search engine with the \textit{semantic-consistent but promotional} texts. To the best of our knowledge, it is the first study of this kind.
% 
\zlccs{Also importantly, when applied to Wiki search poisoning, our approach outperforms all of the state-of-the-art adversarial text ranking attack approaches~\cite{song2020adversarial,liu2022order,wu2022prada} in both effectiveness and efficiency (see Sections~\ref{subsec:promotionEffective}, ~\ref{subsec:userstudy}, and~\ref{sec:abla}).}



